A Multivariate Statistical Analysis of Spiral Galaxy Luminosities. II. Morphology-Dependent Multiwavelength Emission Properties

This is the second of two papers based on a systematic multi-wavelength (X, B, H, 12$\mu$m, FIR, 6cm) statistical analysis of the {\it Einstein Observatory Galaxy Catalog} sample of 234 `normal' S0/a-Irr galaxies. This sample is representative of spiral galaxies (Paper I), and its wide wavelength coverage provides a unique opportunity for a systematic exploration of the relations among different emission bands, that can give novel insight on the different emission processes and their relation to galaxian components, as a function of galaxy morphology.

==> table1.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother



\begin{deluxetable}{lrrrrrrr}
\tablenum{1}
\tablewidth{0pc}
\tablecaption{Residuals For Early and Late Samples}
\tablehead{
\colhead{Pair (Y, X)} &
\colhead{Mean Residual} &
\colhead{Mean Residual} &
\colhead{Prob 1 \tablenotemark{a}}&
\colhead{Prob 2 \tablenotemark{b}}&
\colhead{Prob 3 \tablenotemark{c}}&
\colhead{Prob 4 \tablenotemark{d}}&
\colhead{Prob 5 \tablenotemark{e}} 
  \\
\colhead{} &
\colhead{$T = 5 - 10$} &
\colhead{$T = 0 - 2$} &
\colhead{}&
\colhead{}&
\colhead{}&
\colhead{}&
\colhead{}
  \\
}
\startdata

B,X & -0.147 $\pm$  0.046 & -0.206 $\pm$  0.044 & 0.7961 & 0.7932 &  0.2520 & 0.4899 & 0.4918\nl

X,B &  0.217 $\pm$  0.068 &  0.304 $\pm$  0.065 & 0.7961 & 0.7932 &  0.2520 & 0.4899 & 0.4918\nl
& & & & & & & \nl

B,H &  0.011 $\pm$  0.024 & -0.260 $\pm$  0.028 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & \nodata\nl

H,B & -0.016 $\pm$  0.033 &  0.355 $\pm$  0.038 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & \nodata\nl
& & & & & & & \nl

B,12 & -0.109 $\pm$  0.035 &  0.009 $\pm$  0.059 & 0.1108 & 0.1199 &  0.0602 & 0.0623 & 0.0623\nl

12,B &  0.243 $\pm$  0.077 & -0.018 $\pm$  0.132 & 0.1108 & 0.1199 &  0.0602 & 0.0623 & 0.0623\nl
& & & & & & & \nl

B,FIR &  0.000 $\pm$  0.027 &  0.392 $\pm$  0.068 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl

FIR,B &  0.003 $\pm$  0.041 & -0.591 $\pm$  0.102 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl
& & & & & & & \nl

B,6cm & -0.029 $\pm$  0.066 &  0.412 $\pm$  0.103 & 0.0008 & 0.0008 &  0.0001 & 0.0004 & 0.0002\nl

6cm,B &  0.048 $\pm$  0.107 & -0.659 $\pm$  0.165 & 0.0008 & 0.0008 &  0.0001 & 0.0004 & 0.0002\nl
& & & & & & & \nl

H,X & -0.044 $\pm$  0.086 &  0.190 $\pm$  0.075 & 0.0092 & 0.0114 &  0.0158 & 0.0055 & 0.0051\nl

X,H &  0.051 $\pm$  0.104 & -0.230 $\pm$  0.090 & 0.0092 & 0.0114 &  0.0158 & 0.0055 & 0.0051\nl
& & & & & & & \nl

H,12 & -0.001 $\pm$  0.064 &  0.497 $\pm$  0.079 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl

12,H &  0.001 $\pm$  0.106 & -0.832 $\pm$  0.132 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl
& & & & & & & \nl

H,FIR & -0.047 $\pm$  0.045 &  0.898 $\pm$  0.108 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl

FIR,H &  0.054 $\pm$  0.054 & -1.067 $\pm$  0.129 & 0.0000 & 0.0000 &  0.0000 & 0.0000 & 0.0000\nl
& & & & & & & \nl

H,6cm & -0.017 $\pm$  0.100 &  0.832 $\pm$  0.160 & 0.0001 & 0.0001 &  0.0000 & 0.0001 & 0.0000\nl

6cm,H &  0.022 $\pm$  0.125 & -1.040 $\pm$  0.200 & 0.0001 & 0.0001 &  0.0000 & 0.0001 & 0.0000\nl
& & & & & & & \nl

\tablenotetext{a}{Probability that early- and late-type distributions 
of residuals are drawn from the same parent population,
using Gehan's Generalized Wilcoxon Test - Permutation Variance method.}

\tablenotetext{b}{Same as a, but according to Gehan's Generalized 
Wilcoxon Test - Hypergeometric Variance method.}

\tablenotetext{c}{Same as a, except using Logrank Test method.}

\tablenotetext{d}{Same as a, except using first Peto \& Peto Generalized Wilcoxon Test method.}

\tablenotetext{e}{Same as a, but according to Peto \& Prentice Generalized 
Wilcoxon Test method. In the absence of censored
data (as in the B,H pair), the Peto \& Prentice test reduces to
Gehan's Generalized Wilcoxon Test. }

\enddata
\end{deluxetable}


==> table2.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother


\begin{deluxetable}{ccrrrrrr}
\tablenum{2}
\tablewidth{0pc}
\tablecaption{Schmitt's Method Regression Bisectors,
$T = 5 - 10$ Sample}
\tablehead{
\colhead{} & \colhead{} &
\colhead{} & \colhead{} &
\colhead{}  &
\multicolumn{3}{c}{Blue Dwarves Removed} \\
\colhead{X} & \colhead{Y} &
\colhead{Slope} & \colhead{$\sigma_{S}$} &
\colhead{Int.}  &
\colhead{Slope\tablenotemark{a}} & \colhead{$\sigma_{S}$\tablenotemark{a}} &
\colhead{Int.\tablenotemark{a}}  \\
 }

\startdata


$L_B$ & $L_X$ &   1.48 &   0.13 & -23.61 &    1.44 &   0.14 & -21.81 \nl
  &  &  &  &  &   &  &  \nl
 
$L_H$ & $L_X$ &   1.20 &   0.13 & -12.03 &    1.09 &   0.13 &  -7.05 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{12}$ & $L_X$ &   0.66 &   0.06 &  12.26 &    0.81 &   0.07 &   5.75 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{FIR}$ & $L_X$ &   0.96 &   0.06 &  -1.60 &    1.00 &   0.07 &  -3.42 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{6cm}$ & $L_X$ &   0.90 &   0.07 &   7.70 &    0.79 &   0.06 &  11.81 \nl
  &  &  &  &  &   &  &  \nl
 
$L_H$ & $L_B$ &   0.73 &   0.04 &  11.34 &    0.74 &   0.05 &  10.87 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{12}$ & $L_B$ &   0.45 &   0.04 &  23.99 &    0.60 &   0.04 &  17.40 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{FIR}$ & $L_B$ &   0.66 &   0.04 &  14.34 &    0.67 &   0.05 &  13.80 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{6cm}$ & $L_B$ &   0.62 &   0.07 &  20.64 &    0.61 &   0.07 &  21.03 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{12}$ & $L_H$ &   0.60 &   0.05 &  17.89 &    0.75 &   0.07 &  11.45 \nl
  &  &  &  &  &   &  &  \nl
 
$L_H$ & $L_{FIR}$ &   1.19 &   0.09 &  -7.99 &    1.15 &   0.11 &  -6.27 \nl
  &  &  &  &  &   &  &  \nl
 
$L_H$ & $L_{6cm}$ &   1.25 &   0.23 & -18.27 &    1.25 &   0.20 & -18.27 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{12}$ & $L_{FIR}$ &   0.74 &   0.03 &  11.99 &    0.86 &   0.03 &   6.91 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{12}$ & $L_{6cm}$ &   0.88 &   0.07 &  -1.37 &    0.98 &   0.08 &  -5.66 \nl
  &  &  &  &  &   &  &  \nl
 
$L_{6cm}$ & $L_{FIR}$ &   0.91 &   0.06 &  10.67 &    0.87 &   0.04 &  12.23 \nl
  &  &  &  &  &   &  &  \nl
 
\tablenotetext{a}{ Regression coefficients computed with blue dwarf
galaxies excluded.
Galaxies removed from the sample for this analysis are: NGC 6822, SMC,
NGC 4236, IC 2574, NGC 4244, NGC 247, IC 1613. These blue late-type
dwarf galaxies appear as a distinct population in Fig. 8, possibly
indicating an ISM composition different from more luminous
systems. We omit the blue dwarfs from the sample to study their
effect on the regression results.
}
\enddata
\end{deluxetable}

